Guaranteed Feasibility in Differentially Private Linearly Constrained Convex Optimization

Convex programming with linear constraints plays an important role in the operation of a number of everyday systems. However, absent any additional protections, revealing or acting on the solutions to such problems may reveal information about their constraints, which can be sensitive. Therefore, in this paper, we introduce a method for solving convex programs while keeping linear constraints private. First, we prove that this method is differentially private and always generates a feasible optimization problem (i.e., one whose solution exists). Then we show that the solution to the privatized problem also satisfies the original, non-private constraints. Next, we bound the expected loss in performance from privacy, which is measured by comparing the cost with privacy to that without privacy. Simulation results apply this framework to constrained policy synthesis in a Markov decision process, and they show that a typical privacy implementation induces only an approximately $9\%$ loss in solution quality.

==> Figures/algorithm_flowchart.tex <==
\tikzstyle{start} = [rectangle, rounded corners, 
minimum width=3cm, 
minimum height=1cm,
text centered, 
draw=black, 
fill=red!30]

\tikzstyle{stop} = [rectangle, rounded corners, 
minimum width=3cm, 
minimum height=1cm,
text centered, 
draw=black, 
fill=green!30]

\tikzstyle{io} = [trapezium, 
trapezium stretches=true, % A later addition
trapezium left angle=70, 
trapezium right angle=110, 
minimum width=3cm, 
minimum height=1cm, text centered, 
draw=black, fill=blue!30]

\tikzstyle{process} = [rectangle, 
minimum width=3cm, 
minimum height=1cm, 
text centered, 
text width=3cm, 
draw=black, 
fill=yellow!30]

\tikzstyle{decision} = [diamond, 
minimum width=3cm, 
minimum height=1cm, 
text centered, 
draw=black, 
fill=green!30]

\tikzstyle{arrow} = [thick,->,>=stealth]
\begin{tikzpicture}
%[node distance=4.5cm]

\node (start) [start] {Determine~$A$};
\node (pro2) [process, right= 0.5cm of start] {Privatize the non-zero entries in each row of~$A,~a^0_{i,j}$, to obtain~$\tilde{a}^0_{i,j}$};
\node (pro3) [process, right= 0.5cm of pro2] {Post-process~$\tilde{a}^0_{i,j}$ to obtain $\bar{a}^{0}_{i,j}$ and form~$\tilde{A}$};
\node (finish) [stop, right= 0.5cm of pro3] {Solve Problem~\ref{opt:DP} to obtain~$\tilde{x}^*$};


\draw [arrow] (start) -- (pro2);
\draw [arrow] (pro2) -- (pro3);
\draw [arrow] (pro3) -- (finish);



\end{tikzpicture}
